Powering COVID-19 community Q&A with Curated Side Information

Community question answering and discussion platforms such as Reddit, Yahoo! answers or Quora provide users the flexibility of asking open ended questions to a large audience, and replies to such questions maybe useful both to the user and the community on certain topics such as health, sports or finance. Given the recent events around COVID-19, some of these platforms have attracted 2000+ questions from users about several aspects associated with the disease. Given the impact of this disease on general public, in this work we investigate ways to improve the ranking of user generated answers on COVID-19. We specifically explore the utility of external technical sources of side information (such as CDC guidelines or WHO FAQs) in improving answer ranking on such platforms. We found that ranking user answers based on question-answer similarity is not sufficient, and existing models cannot effectively exploit external (side) information. In this work, we demonstrate the effectiveness of different attention based neural models that can directly exploit side information available in technical documents or verified forums (e.g., research publications on COVID-19 or WHO website). Augmented with a temperature mechanism, the attention based neural models can selectively determine the relevance of side information for a given user question, while ranking answers.

==> comment.tex <==
\begin{comment}
\begin{table}[t]
\begin{tabular}{|l|l|l|}\hline
Stat &  TREC & WHO \\ \hline 
Q-(A/D) pairs &5099 & 147\\ \hline
#qwords & & 13.28$\pm$5.36\\ \hline
#awords & & \\ \hline
\end{tabular}
\caption{Data from external sources}
\label{table:external_stat}
\end{table}

\end{comment}


\begin{comment}
\begin{table}[t]
\scalebox{0.8}{
\begin{tabular}{|l||l|l|l||l|l|l|}\hline
\multirow{2}{*}{Primary} & \multicolumn{3}{|c|}{Train} &\multicolumn{3}{|c|}{Test} \\
& Q-A &\#qwords & \#awords & Q-A &\#qwords & \#awords \\ \hline
Yahoo! Ans & & & & & & & \\ \hline 
Infobot & & & & & & & \\  \hline \hline
\multirow{2}{*}{Primary} & \multicolumn{3}{|c|}{Train} &\multicolumn{3}{|c|}{Test} \\
& Q-A &\#qwords & \#awords & Q-A &\#qwords & \#awords \\ \hline

\end{tabular}}
\caption{Train and test statistics}
\label{table:train_test_stat}
\end{table}
\end{comment}

\begin{comment}
\begin{table}[t]
\begin{tabular}{|l|l|l||l|l|}\hline
 & \multicolumn{2}{|c|}{Yahoo! Ans}  & \multicolumn{2}{|c|}{EMNLP}  \\ \hline
Model & P$@$1 & R$@$3  & P$@$1 & R$@$3    \\ \hline
$\tau$-att-0.25	&	0.435	& 0.718 & 0.722 & 0.852 \\ \hline
$\tau$-att-0.50	&	0.36	&	0.66 & 0.656 & 0.837 \\ \hline
$\tau$-att-0.75	&   0.31	&  0.494 & 0.526 & 0.813 \\ \hline
$\tau$-att-1.0	&	0.33	&	0.59  & 0.698 & 0.859\\\hline
$\tau$-att-2.0	&	0.32	&	0.56  & 0.504  & 0.790 \\\hline
$\tau$-att-5.0	&	0.339	&	0.59  & 0.573 & 0.790\\\hline
$\tau$-att-10.0	&	0.318	&	0.58  & 0.581 & 0.795 \\\hline
$\lambda$-sim-0.5 & 0.304 & 0.58  & 0.537  & 0.782 \\\hline
$\lambda$-sim-1.0 & 0.30 & 0.55  & 0.332 & 0.630\\ \hline
$\lambda$-sim-0.75 & 0.299 & 0.57  &0.457 & 0.712\\\hline
bert-sl256 & 0.406 & 0.657 & & \\ \hline
bert-sl128 & 0.363 & 0.604 & & \\ \hline
ques-att \cite{} & & & &\\ \hline
lstm \cite{} & & & &\\ \hline
cnn+lstm \cite{} & & & &\\ \hline
%tqsim & 0.28 & 0.53 \\ \hline
$\lambda$-sim-0.25 & 0.27 & 0.56  & 0.541& 0.798\\\hline
qasim & 0.26 & 0.57  & 0.542  & 0.809\\ \hline
random & 0.21 &   &  0.239 &\\ \hline
\end{tabular}
\caption{Precision and Recall for different models}
\label{table:prec_recall}
\end{table}
\end{comment}

==> sections/method_old.tex <==
\section{Method} \label{sec:method}

\subsection{Problem formulation}

For this task, our dataset consists of $n$ questions $q_1, \ldots, q_n$
related to COVID-19. Each $q_i$ is associated with a set of two or more answers
$A_i = \{a_{ij}: 2 \le j\}$ and corresponding labels 
$Y_i = \{y_{ij}: 2 \le j\}$ representing answer relevance. Labels may
be defined as either:
\begin{itemize}
    \item Binary relevant judgments (e.g., \textit{favorite}, \textit{selected}) provided by the questioner, i.e., $y_{ij} \in \{0, 1\}$
    \item Integers representing aggregated votes provided by the community, i.e., $y_{ij} \in \mathbb{Z}$.
\end{itemize}
We attempt to model the relevance of each answer $a_{ij}$ to its corresponding
question using an external knowledge base consisting of information-seeking
queries $r_1, \ldots, r_m$ related to COVID-19, with each $r_k$ linked to a set of
relevant scientific articles $S_k$ as determined by human judges for the TREC task.
Query text can be expanded to include alternative formulations such as a question
or a short narrative describing the informational goals of the searcher.
\kapil{insert table with sample data}

We hypothesize that this knowledge base of scientific literature may be valuable
in identifying answer quality for certain kinds of questions, although not all.
We investigate this by experimenting with models to recover the true labels
$y_{ij}$ for each answer
$a_{ij} \in A_i$ given its question $q_i$, category information, and the
full knowledge base $\langle r_k, S_k \rangle_{k=1}^m$.

\subsection{Model}

In this work, we explore data-efficient matching mechanisms to determine the
relevance of articles in the knowledge base that may inform the label prediction
task.
First, the question $q_i$, an answer $a_{ij}$ and additional metadata can be
encoded into a $d$-dimensional vector $x_i$ using a pretrained text encoder
$f_\text{input}$.
\begin{align*}
    x_{ij} &= f_\text{input}(q_i, a_{ij})
\end{align*}
%If no side information was available, this vector would normally be supplied
%directly to a label prediction network $g$.
%\begin{align*}
%    \hat{y}_{ij} &= g(x_{ij})
%\end{align*}
In order to incorporate side information, each expanded query $r_k$ and
corresponding collection of scientific abstracts $S_k$ from the TREC dataset are
also encoded into vectors using pretrained encoders.
\begin{align*}
    p_k &= f_\text{query}(r_k) \\
    s_k &= f_\text{docs}(S_k)
\end{align*}
Here, $f_\text{query}$ may be the same generic encoder as $f_\text{input}$ or a
different encoder that produces $d$-dimensional embeddings. In
contrast, $f_\text{docs}$ should be adapted to scientific literature, so we
produce abstract embeddings using BioBERT and combine the embeddings of the
most query-relevant documents.
\kapil{note that an average may be too coarse here.}

We condition on this side information using a variant of scaled dot-product
attention, which provides a straightforward conditioning approach over a set of
query-document pairs. Input vector $x_{ij}$ serves as a query over keys
$p_k$ to determine the relevance of each corresponding $s_k$.
Each vector is linearly projected prior to this computation within
$f_\text{input}, f_\text{query}, f_\text{docs}$ respectively.
\begin{align*}
    z_k &= \frac{x_{ij}^\top p_k}{\sqrt{d}} \\
    \alpha_{ijk} &= \frac{e^{z_k/t}}{\sum_l e^{z_l/t}} \\
    s_{ij}' &= \sum_k \alpha_{ijk} s_k
\end{align*}
where $t$ is a temperature term to control the uniformity of attention weights
$\alpha_k$. Finally, labels are predicted using a
multi-layer perceptron over the input vector $x_{ij}$ and the learned weighted
average of side information $s_{ij}'$.
\begin{align*}
    \hat{y}_{ij} &= f_\text{output}([x_{ij}; s_{ij}'])
\end{align*}
where $f_\text{output}$ contains leaky ReLU activation functions. 

\subsection{Gating side-information}

As the questions in our dataset may often be entirely unrelated to scientific
literature, a key aspect of this approach is determining \textit{whether}
the TREC side information is useful, not merely attending to \textit{which}
queries are most relevant. We consider two strategies for achieving this:
\begin{enumerate}
    \item Learning a softmax temperature parameter $t$ as a function of $x_{ij}$
        in the attention mechanism, which can prevent the softmax operation from
        concentrating attention weights for non-scientific questions.
        \begin{align*}
            t &= f_\text{temp}(x_{ij})
        \end{align*}
    \item Adding a dummy entry $\langle r_{m+1}, \S_{m+1} \rangle$ to the side
        information where the corresponding $s_{m+1}$ is a zero vector that
        produces no activations within $f_\text{output}$.
\end{enumerate}

==> sections/related_old.tex <==
\section{Related work} \label{sec:related}
In the section we cover related work on QA, and COVID-19 inspired retrieval tasks.

\subsection{QA on unstructured knowledge bases}
BioBERT \cite{BioBERT}


\subsection{COVID-19 inspired retrieval tasks}
TREC \cite{TREC_covid}. In \cite{jimmy_lin_covid_qa}, a search engine that exploits state-of-the-art neural ranking architectures was introduced to facilitate access to the COVID-19 Open Research Dataset curated
by the Allen Institute for AI.

COVID-19 QA \cite{cairecovid}.
Knowledge search \cite{sledge_scibert}.

% https://www.aaai.org/ocs/index.php/AAAI/AAAI18/paper/download/17226/16146

% https://arxiv.org/pdf/1905.02019.pdf
% student report (perhaps not relevant) https://web.stanford.edu/class/archive/cs/cs224n/cs224n.1174/reports/2761224.pdf
% https://dl.acm.org/doi/10.1145/3077136.3080699 [sigir short position]
% https://dl.acm.org/doi/10.1145/3209978.3210081 [sigir short KB]
% https://dl.acm.org/doi/pdf/10.1145/3184558.3191830 [www short]
% https://dl.acm.org/doi/pdf/10.1145/3308558.3313518 [www short]
% https://www.aclweb.org/anthology/P16-1122.pdf
% https://www.aclweb.org/anthology/D18-1240.pdf 
% https://www.aclweb.org/anthology/C18-1279.pdf (CICLING)
% https://www.aclweb.org/anthology/C18-1215.pdf (CICLING)
% https://arxiv.org/pdf/1905.10720.pdf [arxiv long]

